Object Priors for Classifying and Localizing Unseen Actions

This work strives for the classification and localization of human actions in videos, without the need for any labeled video training examples. Where existing work relies on transferring global attribute or object information from seen to unseen action videos, we seek to classify and spatio-temporally localize unseen actions in videos from image-based object information only. We propose three spatial object priors, which encode local person and object detectors along with their spatial relations. On top we introduce three semantic object priors, which extend semantic matching through word embeddings with three simple functions that tackle semantic ambiguity, object discrimination, and object naming. A video embedding combines the spatial and semantic object priors. It enables us to introduce a new video retrieval task that retrieves action tubes in video collections based on user-specified objects, spatial relations, and object size. Experimental evaluation on five action datasets shows the importance of spatial and semantic object priors for unseen actions. We find that persons and objects have preferred spatial relations that benefit unseen action localization, while using multiple languages and simple object filtering directly improves semantic matching, leading to state-of-the-art results for both unseen action classification and localization.

==> old/abstract-old.tex <==
\begin{abstract}
This work strives for spatio-temporal localization and classification of actions in videos, without the need for labeled training examples. The main contribution is an object embedding that models the spatial and semantic relation between actions and objects. We propose a spatial-aware matching function that takes into account the spatial relations of actors and objects from object detection datasets. The spatial-awareness emphasizes locations in test videos where actors and objects have spatial co-occurence as expected from prior knowledge. We also introduce semantic-aware matching functions able to deal with semantic ambiguity, non-discriminative objects, and the varying levels of precision of object categories. Lastly, we incorporate information about global objects from context as further evidence of the presence of actions in videos. Next to zero-shot action classification and localization, our embedding allows for spatio-temporal action retrieval based on composite queries containing objects as well as their positions and sizes. Experimental evaluation on four action datasets shows the importance of semantic-, spatial-, and global-awareness in zero-shot action localization and classification, where we obtain state-of-the-art results.
\end{abstract}

==> old/conclusions-old.tex <==
\section{Conclusions}
\label{sec:conclusions}

==> old/experiments-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SETUP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental setup}
\label{sec:setup}

\subsection{Datasets}
We evaluate our approach on four datasets, namely UCF Sports~\citep{rodriguez2008action}, J-HMDB~\citep{jhuang2013towards}, UCF-101~\citep{soomro2012ucf101}, and Hollywood2Tubes~\citep{mettes2016spot}.

\textbf{UCF Sports} contains 150 videos from 10 actions such as \emph{Running} and \emph{Horse Riding}~\citep{rodriguez2008action}. The videos are from sports broadcasts. We employ the train/test split provided by~\citep{lan2011discriminative}.

\textbf{J-HMDB} contains 928 videos from 21 actions such as \emph{Brushing hair} and \emph{Catching}~\citep{jhuang2013towards}. The videos focus on daily human activities. We employ the train/test split provided by~\citep{jhuang2013towards}.

\textbf{UCF-101} contains 3,207 videos from 24 actions such as \emph{Skiing} and \emph{Playing Basketball}~\citep{soomro2012ucf101}. The videos contain both sports and daily activities. We employ the train/test split provided by~\citep{soomro2012ucf101}.

\textbf{Hollywood2Tubes} contains 1,707 videos from 12 actions of Hollywood2~\citep{marszalek09}, which contain video clips from movies. The dataset is supplemented with spatio-temporal localization annotations by~\citep{mettes2016spot}. We employ the train/test split provided by~\citep{marszalek09}.

For all datasets, we exclude the use of any information from the training videos. We employ the action labels and ground truth box annotations from the test videos to evaluate our zero-shot action localization and classification.

\subsection{Prior knowledge}
To obtain person and object box detections in frames, we employ Faster R-CNN~\citep{ren2015faster}, pre-trained on MS-COCO~\citep{lin2014microsoft}. The pre-trained network includes the person class and 79 objects, such as \emph{car}, \emph{chair}, and \emph{tv}. For the global object scores, we employ a GoogLeNet~\citep{szegedy2015going}, pre-trained on 12,988 ImageNet categories~\citep{mettes2016imagenet}.

For the spatial relations, we reuse the bounding box annotations of the training set of MS-COCO, readily used to pre-train the detection model, to obtain the expected spatial awareness between persons and objects.

For the semantic relations, we investigate the use of two pre-trained word embedding models. The first is a word2vec model~\citep{mikolov2013distributed}, pre-trained on metadata of the images and videos from the YFCC100M dataset~\citep{thomee2015yfcc100m}, akin to the zero-shot action recognition of~\cite{jain2015objects2action}. The second is FastText, pre-trained on 157 languages~\citep{grave2018learning}. This collection of word embeddings enables us to investigate multi-lingual semantic matching between actions and objects. For the multi-lingual experiments, we employ five languages: English, French, Dutch, Italian, and Afrikaans. We obtain action and object translations first from \psmm{multi-lingual WordNet~\citep{?}.} For the remaining objects and the actions, we use Google Translate with manual verification.

\subsection{Implementation details}

\subsection{Evaluation protocol}
We follow the zero-shot action setup of~\citep{jain2015objects2action,mettes2017spatial,zhu2018towards}, where no training is performed on a separate set of actions; the set of test actions are directly evaluated. For each dataset, we evaluate on the videos in the test set. For the experiments where we use fewer test action than the total number of actions, we perform a random selection of test actions.

For zero-shot action localization, we compute the spatio-temporal (st) overlap between action tube $a$ and ground truth $b$ from the same video as: $\text{st-iou}(a,b) = \frac{1}{|\Gamma|} \sum_{f \in \Gamma} \text{iou}_f(a,b)$, where $\Gamma$ states the union of frames in $a$ and $b$. The function $\text{iou}_f(a,b)$ is 0 if either one of the tubes is not present in frame $f$. For overlap threshold $\tau$, an action tube is positive if the tube is from a positive video, the overlap with a ground truth instances is at least $\tau$, and the ground truth instance has not been detected before. We use mAP and AUC for evaluation, following the convention in the literature \citep{?,?,?}.

For zero-shot action classification, we evaluate using multi-class classification accuracy.

\begin{table*}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
 & \multicolumn{5}{c}{Localization} & \multicolumn{5}{c}{Classification}\\
nr. local objects & 0 & 1 & 2 & 5 & 10 & 0 & 1 & 2 & 5 & 10\\
\midrule
Person & 10.1 & - & - & - & - & 8.5 & - & - & - & -\\
+ Objects & - & \textbf{23.2} & 21.9 & 21.6 & 21.5 & - & 21.8 & 14.9 & 19.2 & 12.8\\
\rowcolor{Gray}
+ Spatial relations & - & \textbf{23.2} & 22.8 & 21.4 & 22.3 & - & 21.3 & 23.4 & \textbf{25.5} & 17.0\\
\bottomrule
\end{tabular}
\caption{Effect of local objects and spatial relations on the localization (mAP@0.5, \%) and classification (acc, \%) results for UCF Sports. We investigate three variants of our local object embeddings; one using only person detections, one using person and object detections, and one with the additional spatial relations between people and objects. We find that for localization, using only one object is preferred, while for classification more objects result in higher scores.}
\label{tab:study1}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental results}
\label{sec:results}

\subsection{The effect of objects and spatial relations}
In the first experiment, we investigate zero-shot action classification and localization using only our local object embeddings. We evaluate the effect of the use of local objects and spatial relations between people and objects. Additionally, we investigate how many objects per action are desirable in our embedding. The localization and classification results for UCF Sports are shown in Table~\ref{tab:study1}.

The results show that when using person detections only (row 1), results near random performance are obtained. This is hardly surprising, since all actions in the dataset are person-centric, hence there is no way to distinguish actions. The addition of objects (row 2) results in a considerable increase in both localization and classification scores, highlighting the importance of using objects to recognize unseen actions.

The addition of spatial relations (row 3) further boosts the scores across different numbers of selected local objects per action. For localization, spatial relations boost the scores for the top 2 and top 10 objects per action. For classification, spatial relations boost the scores for the top 2, 5, and 10 objects per action. This result indicates that spatial relations provide additional information for unseen actions.

Overall, we find that the preferred number of objects per action varies per task. For localization, only one object per action is preferred, while five objects per action are preferred for classification. A reason for lower localization scores with more objects is that people are more likely to interact with a single object, at least in the UCF Sports dataset. For classification, more object are preferred. This indicate that for classification, we want to aggregate more information about object presence in videos, rather than exploit the single most relevant object per action. This is because a precise overlap between the spatio-temporal and ground truth localization tubes is no longer required; a global video score is sufficient.

We conclude from this experiment that local objects and spatial relations matter for both zero-shot action localization and classification. We will therefore rely on both aspects in further experiments.

\subsection{Evaluating global embeddings}

\subsection{Zero-shot localized action retrieval}

\subsection{State-of-the-art comparison}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 & \multicolumn{5}{c}{Overlap threshold}\\
 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5\\
\midrule
\rowcolor{Gray}
Fully supervised & & & & &\\
\cite{weinzaepfel2015learning} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\midrule
\rowcolor{Gray}
Weakly-supervised & & & & &\\
\cite{mettes2017localizing} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\midrule
\rowcolor{Gray}
Zero-shot & & & & &\\
\cite{jain2015objects2action} & 00.0 & 00.00 & 00.0 & 00.0 & 00.0\\
This paper & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\bottomrule
\end{tabular}
}
\caption{Comparative evaluation of action localization on UCF Sports using the AUC metric. \psmm{observations and conclusions.}}
\label{exp:sota-localization-1}
\end{table}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 & \multicolumn{5}{c}{Overlap threshold}\\
 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5\\
\midrule
UCF-101-24 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
J-HMDB & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
Hollywood2Tubes & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\bottomrule
\end{tabular}
}
\caption{First zero-shot action localization results on UCF-101-24, J-HMDB, and Hollywood2Tubes with the AUC metric. No direct zero-shot comparison is available for these datasets, hence these results serve as baselines for future investigations. \psmm{observations and conclusions.}}
\label{exp:sota-localization-2}
\end{table}

==> old/introduction-old.tex <==
\section{Introduction}
The goal of this paper is to localize and classify human actions in videos. Both action tasks are actively researched topic in computer vision, with approaches based on two-stream networks~\citep{simonyan2014two,kalogeiton2017action}, recurrent networks \citep{veeriah2015differential,li2018videolstm}, and 3D convolutional networks~\citep{carreira2017quo,hou2017tube}. Common among these works is the need for video examples during training. Localization even requires spatio-temporal annotations within the videos. Obtaining video examples and spatio-temporal annotations is however expensive and prohibitive, limiting the applicability and scalability of current works. In this paper, we aim to acquire a localization and classification of actions without the need for \emph{any} video examples during training.

\begin{figure}[t]
\centering
\textcolor{Gray}{\rule{8cm}{5cm}}
\caption{TO DO.}
\label{fig:fig1}
\end{figure}

In zero-shot action recognition, the common setup is to obtain action scores by performing a semantic match with pre-defined attributes~\citep{?,?,?}, object classifications~\citep{?,?,?}, or seen training actions~\citep{?,?}. While intuitive for classification, these approaches are neither capable nor intended to determine the precise action location, as all visual information is captured at the frame or video level. Furthermore, current works employ standard word models for the semantic matching, ignoring persistent linguistic gaps between actions and objects. In this paper, we propose object embeddings for unseen actions that integrate both an awareness for spatial and semantic relations between actions and objects, enabling effective spatio-temporal action localization and classification directly from objects. Figure~\ref{fig:fig1} highlights our main notions.

For a spatial awareness in our embedding, we posit that people and objects occur in preferred spatial relations. For example, a skateboard is below someone \emph{skateboarding}, a baseball bat is to the left or right of someone \emph{playing baseball}, and a traffic light is above someone \emph{crossing the road}. To encode such information without action examples, we start from existing object detection datasets and models. Box annotations in object datasets allow us to assess how people and objects are commonly related spatially. From discovered spatial relations, we propose a score function that combines person detections, object detections, and their spatial match for unseen action localization and classification.

Next to spatial relation, we also investigate the semantic matching between actions and objects, a vital aspect when training examples are absent. We investigate several persistent linguistic gaps in the semantic matching. The first gap is semantic ambiguity. Both action and object names can have multiple meanings, which can result in an incorrect matching between activities and objects. To alleviate this effect, we perform multi-lingual semantic matching, inspired by the linguistic principle that objects are coherent across languages and cultures~\citep{malt1995}. The second gap is the selection of semantically relevant but non-discriminative objects. We introduce two relevance functions to estimate which objects are most exclusive, thus most discriminant, for an action in order to emphasize these in the matching process. The third gap is determining which level of object description is desirable for matching to actions. A well-known principle is that of basic-level objects, which correspond to an intermediate level of description~\citep{rosch1976,rosch1988}, which provides the most specific information when naming an object. Here, we investigate whether it is important to focus on basic-level objects for unseen action localization and classification.

%To alleviate the effect of semantic ambiguity, we take inspiration from the linguistic principle that objects are coherent across languages and cultures~\citep{malt1995}. We leverage this principle by investigating multi-lingual unseen action recognition. The second gap is the selection of semantically relevant but non-discriminative objects. We take inspiration from the principle of object taxonomies, which indicate the shareability and the exclusiveness of objects~\citep{rosch1976,murphy2004big}. We introduce two relevance functions to estimate which objects are most exclusive, thus most discriminant, for an action in order to emphasize these in the matching process. The third gap is determining which level of object description is desirable for matching to actions. A well-known principle is the notion of basic-level objects. It corresponds to an intermediate level of description~\citep{rosch1976,rosch1988}, which provides the most specific information when naming an object. Here, we investigate whether it is important to focus on basic-level objects for unseen action localization and classification.

Beyond local object embeddings for unseen actions, we show how to incorporate global objects from context to improve both localization and classification. Lastly, due to the general nature of our approach, we introduce a new task: zero-shot localized action retrieval, where spatio-temporal action locations are obtained from a dataset, based on user queries specifying desired objects, object sizes, and spatial relations. Experiments on four action datasets show the importance of focusing on spatial awareness, semantic awareness, and global objects for unseen action localization and classification. Our approach obtains state-of-the-art zero-shot results for tasks, highlighting its effectiveness and more generally, emphasizing the strong link between actions and objects.

The rest of the paper is organized as follows. Section~\ref{sec:related} discusses related work. Section~\ref{sec:embedding} provides an overview of the object embeddings for unseen actions, along with the spatial and semantic components of the embeddings.%, while Section~\ref{sec:relations} presents the spatial and semantic components of the embeddings.
Section~\ref{sec:global} discusses the inclusion of global objects and Section~\ref{sec:retrieval} introduces the zero-shot localized action retrieval task. Sections~\ref{sec:setup} and~\ref{sec:results} discuss respectively the experimental setup and results. The paper is concluded in Section~\ref{sec:conclusions}.

==> old/method-old-v0.tex <==
\section{Object embeddings for unseen actions}
For zero-shot action localization and classification, we are given a set of action class names $\mathcal{Z} = \{z_{1},..,z_{c}\}$ from $c$ action categories.
We do not assume any action examples for training, neither from $\mathcal{Z}$ or from a disjoint set of action categories. Therefore, we directly bypass the training stage. During testing, we are given a set of test videos $\mathcal{V}$. For zero-shot action classification, we aim to assign the correct action class to each test video. For zero-shot action localization, we aim to extract spatio-temporal tubes relevant for each action from the test videos. We outline our proposed object embeddings in four steps: (i) semantic matching between actions and objects, (ii) spatial-aware action box scoring, and (iii) action tube linking.

%
% PRIOR KNOWLEDGE
%
\subsection{Prior semantic and object knowledge}
Our zero-shot action approach relies on three sources of prior knowledge. The first is a collection of object detectors from image datasets. Let $\mathcal{O} = \{\mathcal{O}^{(i)}_N, \mathcal{O}^{(i)}_D\}_{i=1}^{n}$ denote respectively the names and detectors for $n$ object classes. We denote $\mathcal{A} = \{\texttt{person}, \mathcal{A}_D\}$ as a person detector. Each detector outputs a set of bounding boxes with corresponding object likelihoods for a given video frame.

The second source is the semantic relations between actions and objects. For now, we map action class names to objects with the use of word embeddings~\citep{mikolov2013distributed}. This setup will be extend in the next section. For an action $z \in \mathcal{Z}$, we compute the semantic similarity to an object $o \in \mathcal{O}$ as:
\begin{equation}
w(o, z) = \text{cos}(e(o_{N}), e(z)),
\end{equation}
where $e(\cdot)$ denotes the embedding of a word into a word embedding space and $\text{cos}(\cdot,\cdot)$ denotes the cosine similarity, \ie $\text{cos}(\textbf{a},\textbf{b}) = \frac{\textbf{a} \cdot \textbf{b}}{||\textbf{a}|| ||\textbf{b}||}$. For actions or objects described by more than one word, we average that word embedding representations of the individual words~\citep{mikolov2013distributed}.

The third source targets the spatial awareness between people and objects. We exploit the observation that people interact with objects in preferred spatial relations. We do this by gathering statistics from the same image dataset used to pre-train the object detectors. By reusing the same dataset, we keep the amount of knowledge sources contained to a dataset for object detectors and a semantic word embedding. For the spatial awareness, we examine the bounding box annotations for the person class and all object classes. We gather all instances where an object and person box annotation co-occur. We quantize the gathered instances into representations that describe the overall spatial-awareness between people and objects. We cluster the representations into a limited number of exemplar spatial relations $\mathcal{E}_o$ for each object $o$.

%
% BOX SCORING
%
\subsection{Spatial-aware action box scoring}
Based on the extracted prior knowledge on objects and their semantic relations to actions, we propose a function that scores individual boxes given any action class name. For a bounding box $b$ in video frame $F$, we define a score function for action class $z$. The score function is proportional to three conditions.
\\\\
\textbf{Condition 1:} \emph{The likelihood of an action class in box} b \emph{is proportional to the likelihood of a person present in} b.
\\\\
The first condition follows directly from our focus on human action recognition. The first condition is independent of the specific action class, as it must hold for any action. The score function therefore adheres to the following:
\begin{equation}
s(b, F, z) \propto Pr(\texttt{person} | b). 
\end{equation}
\textbf{Condition 2:} \emph{The likelihood of action class $z \in \mathcal{Z}$ in box} b \emph{is proportional to the likelihood of detected objects, provided that the detected objects are (i) semantically close to action class $z$ and (ii) the detection is sufficiently close to} b.
\\\\
The second condition states that the presence of an action in a box $b$ also depends on the presence of \emph{relevant} objects in the \emph{vicinity} of $b$. We formalize this as:
\begin{equation}
s(b, F, z) \propto \sum_{o \in \mathcal{O}} w(o, z) \cdot \max_{b' \in o_{D}(F)} \bigg( \delta_s(b, b') \cdot Pr(o_{N} | b') \bigg),
\label{eq:emb-c2}
\end{equation}
\begin{figure}[t]
\centering
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/backpack.pdf}
\caption{Backpack.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/umbrella.pdf}
\caption{Umbrella.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/stop-sign.pdf}
\caption{Stop sign.}
\end{subfigure}
\\
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/sheep.pdf}
\caption{Sheep.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/horse.pdf}
\caption{Horse.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/giraffe.pdf}
\caption{Giraffe.}
\end{subfigure}
\caption{Spatial-aware exemplars for six local objects. Different objects have different spatial preferences with respect to persons. We exploit this spatial awareness for zero-shot action localization.}
\label{fig:exemplars}
\end{figure}
where $o_{D}(F)$ denotes the set of all detections of object $o_{N}$ in frame $F$. Equation~\ref{eq:emb-c2} incorporates action relevancy through the semantic word embedding function $w(\cdot, \cdot)$. The higher the semantic similarity between action $z$ and object $o_{N}$, the higher the score. The vicinity constraint is incorporated through the function $\delta_s(\cdot, \cdot)$. This function is defined as:
\begin{equation}
\delta_s(b, b') =
\begin{cases}
1 & \quad \text{if } \min_{e_1, e_2 \in E(b), E(b')}(e_1, e_2) \leq t_d\\
0 & \quad \text{otherwise,}
\end{cases}
\label{eq:emb-c2-d}
\end{equation}
where $E(\cdot)$ denotes the set of edges for a box.
Equation~\ref{eq:emb-c2-d} ensures that only objects which occur in the vicinity of box $b$ will be considered, where the vicinity is controlled by $t_d$.
\\\\
\textbf{Condition 3:} \emph{The likelihood of action class $z \in \mathcal{Z}$ in box} b \emph{given an object} o \emph{with box detection} d \emph{that abides Assumption 2, is proportional to the match between the spatial awareness of} b \emph{and} d \emph{with the prior spatial awareness of $z$ and} o.
\\\\
The third condition incorporates our notion of spatial-awareness between actions and objects. Our spatial-aware representation computes a spatial distribution between an object and person box.
The spatial relation between an object box relative to a person box is quantized into a 9-dimensional grid. This grid represents represents how the object box is spatially distributed to the person box with respect to the following prepositions: $\{$\emph{above left}, \emph{above}, \emph{above right}, \emph{left}, \emph{on}, \emph{right}, \emph{below left}, \emph{below}, \emph{below right}$\}$. Let $d_{c}(a, b) \in \mathcal{R}^{9}$ denote the spatial distribution of object box $a$ relative to person box $b$. Furthermore, let $\mathcal{E}_o = \{\mathcal{E}_{o}^{(i)}\}_{i=1}^{|\mathcal{E}_o}$ denote the set of exemplar spatial distributions of object $o$ derived from prior knowledge. In Figure~\ref{fig:exemplars}, we show the exemplar distributions of six objects used in our approach. The Figure shows that different objects have different spatial preferences with respect to persons that we exploit for zero-shot human action localization.

For an object $o$ with detection box $a$ that adheres to condition two, the third condition is given as:
\begin{equation}
s(b, F, z) \propto \max_{e \in \mathcal{E}_{o}} - ||e - d_{c}(b, a)||_1.
\end{equation}
So for a relevant object detection, the spatial-aware score given object-person distributions is given as the negative distance of the nearest exemplar distribution.
\\\\
\textbf{Combined box score.}
By combining the three conditions of our spatial-aware object embeddings, we arrive at a final score function for a box given an action. An illustrative overview of the combined equation for an exemplary video frame is shown in Figure~\ref{fig:method-main}. By combining the three conditions into a score function for boxes, we find that the \psmm{color} box in Figure~\ref{fig:method-main} is deemed most relevant for the action \psmm{action}.

%
% TUBE LINKING
%
\subsection{Action tube linking}
Given a score for each box in each frame of test video $V$, we aim to arrive at a spatio-temporal action localization by linking boxes into tubes over time. We link boxes that have high scores from our spatial-aware object embeddings and a have high spatial overlap. Given action $z$ and boxes $b_{1}$ and $b_{2}$ in consecutive frames $F_{1}$ and $F_{2}$, the link score is given as:
\begin{equation}
w(b_{1}, b_{2}, z) = s(b_{1}, F_{1}, z) + s(b_{2}, F_{2}, z) + \text{iou}(b_{1}, b_{2}),
\end{equation}
where $\text{iou}(\cdot, \cdot)$ denotes the spatial intersection-over-union score. We solve the problem of linking boxes into tubes with the Viterbi algorithm~\citep{gkioxari2015finding}. For video $V$, we apply the Viterbi algorithm on the link scores to obtain an action tube. We then remove the used boxes and their links from the video and rerun the Viterbi algorithm on the remaining links to generate a new tube. We reiterate this process until we obtain $T$ tubes. The action score $\ell_z$ for action class $z$ of an action tube $t$ is defined as the average score of the boxes in the tube:
\begin{equation}
\ell_\text{tube}(t, z) = \frac{1}{|t|} \sum_{i=1}^{|t|} s(b_{t_i}, F_{t_i}, z),
\label{eq:tubescore}
\end{equation}
where $b_{t_i}$ and $F_{t_i}$ denote respectively the box and frame of the $i^{\text{th}}$ element in $t$. For zero-shot localization, we gather tubes across all test videos and rank the tubes using the scores provided by Equation~\ref{eq:tubescore}. For zero-shot classification, we disregard the tube locations. For each video, we predict the action class label as the action with the highest tube score within the video.

%
% GLOBAL
%
\subsection{Incorporating global objects}
Next to local object which can help pinpoint when and where actions occur in videos, there are also global objects that provide contextual information. A few examples of such global objects are shown in Figure~\ref{fig:global-examples}. \psmm{highlight two examples.} While global objects do not specify the action location directly, they do provide discriminative information that can help distinguish between videos of heterogeneous actions.
\\\\
\textbf{Global objects.}
Let $\mathcal{G} = \{\mathcal{G}_N^{(i)}, \mathcal{G}_C^{(i)}\}_{i=1}^{m}$ denote a set of $m$ global objects, each with a name and corresponding classifier. Different from the local objects, global objects only provide scores for whole videos. We use the global objects to yield a score for a video $V$ as follows:
\begin{equation}
\ell_\text{global}(V, z) = \sum_{g \in \mathcal{G}} w(g,z) \cdot p(g | V),
\end{equation}
where $w(g,z)$ denotes the semantic relationship score between global object $g$ and action $z$. Variable $p(g | V)$ denotes the probability of global object $g$ being present in video $V$.
\\\\
\textbf{Spatial- and global-aware object embeddings.}
Action localization with local spatial-aware objects and global objects is performed by a linear combination of the two terms for each action tube, \ie:
\begin{equation}
\ell_\text{combined}(t, V, z) = \ell_\text{tube}(t, z) + \ell_\text{global}(V, z).
\end{equation}
The scores from global objects focus on discriminating tubes from different videos while being complementary to local objects. Action classification is done as:
\begin{equation}
c_{V}^{\star}(t_V, V, z) = \argmax_{z \in \mathcal{Z}} \bigg( \max_{t \in t_V} \ell_\text{tube}(t, z) + \ell_\text{global}(V, z) \bigg),
\end{equation}
where $t_V$ denotes all tubes in video $V$.

\section{Semantic-aware object embeddings}

\section{Zero-shot action localization retrieval}

==> old/method-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% METHOD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\textcolor{Gray}{\rule{17cm}{4.5cm}}
\caption{TO DO.}
\label{fig:method1}
\end{figure*}

\section{Object embeddings for unseen actions}
\label{sec:embedding}

\subsection{Setting.}
For zero-shot action localization and classification, we are given a set of action class names $\mathcal{Z} = \{z_{1},..,z_{c}\}$ from $c$ action categories.
We do not assume any action examples for training, neither from $\mathcal{Z}$ or from a disjoint set of action categories. Therefore, we directly bypass the training stage. During testing, we are given a set of test videos $\mathcal{V}$. For zero-shot action classification, we aim to assign the correct action class to each test video. For zero-shot action localization, we aim to extract spatio-temporal action tubes from test videos.

We outline our proposed local object embeddings as follows. In subsection~\ref{sec:m-overview}, we provide the overview of our local object embeddings. In subsection~\ref{sec:m-spatial}, we describe the spatial relation function and in subsection~\ref{sec:m-semantic} we describe our semantic matching functions. Subsection~\ref{sec:m-linking} we outline how to link scored action boxes into spatio-temporal action tubes.
%We outline our proposed object embeddings in three steps: (i) outline of our object embeddings, (ii) incorporating spatial and semantic relations between actions and objects, and (iii) incorporating global object embeddings.
%\wt{comment: should there be links to sections here? btw I feel this paragraph should maybe have its own section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BOX SCORING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Local object embedding overview}
\label{sec:m-overview}
Our zero-shot action pipeline is visualized in Figure~\ref{fig:method1}. For a test video $v \in \mathcal{V}$ and unseen action $z \in \mathcal{Z}$, the first step is to score local boxes in the video with respect to $z$. For a bounding box $b$ in video frame $F$, we define a score function $s(\cdot)$ for action class $z$. The score function is proportional to three conditions.
\\\\
\textbf{Condition 1:} \emph{The likelihood of any action in} b \emph{is proportional to the likelihood of a person present in} b.
\\\\
The first condition follows directly from our setting of human action recognition. The first condition is independent of the specific action class, as it must hold for any action. The score function therefore adheres to the following:
\begin{equation}
s(b, F, z) \propto Pr(\texttt{person} | b). 
\end{equation}
\\
\textbf{Condition 2:} \emph{The likelihood of action class} z {in} b \emph{is proportional to the likelihood of detected objects, provided that the detected objects are (i) semantically close to action class $z$ and (ii) the detection is sufficiently close to} b.
\\\\
The second condition states that the presence of an action in a box $b$ also depends on the presence of \emph{relevant} objects in the \emph{vicinity} of $b$. We formalize this as:
\begin{equation}
s(b, F, z) \propto \sum_{o \in \mathcal{O}} \Psi(o, z) \cdot \max_{b' \in o_{D}(F,b)} Pr(o | b'),
\label{eq:emb-c2}
\end{equation}
where $O$ denotes a set of pre-trained object detectors and $o_{D}(F,b)$ denotes the set of all detections of object $o$ in frame $F$ that are near to box $b$. In practice, this includes all boxes for with the edges are within 50 pixels of $b$, although the localization and classification scores are hardly affected by other settings, as long as the value is smaller than the whole frame. Equation~\ref{eq:emb-c2} incorporates action relevancy through semantic matching function $\Psi(\cdot,\cdot)$, which is detailed in Section~\ref{sec:semantic}. The higher the semantic similarity between action $z$ and object $o$, the higher the score.
\\\\
\textbf{Condition 3:} \emph{The likelihood of action class $z$ in} b \emph{given an object} o \emph{with box detection} d \emph{that abides Assumption 2, is proportional to the match between the spatial awareness of} b \emph{and} d \emph{with the prior spatial awareness of $z$ and} o.
\\\\
The third condition incorporates our notion of spatial-awareness between actions and objects. Our spatial-aware representation computes a spatial distribution between an object and person box. The spatial-aware relation function is given by the function $\Phi(b, d, o)$ and is further detailed in Section~\ref{sec:spatial}.
\\\\
\textbf{Combined score function.} The box score from our object embedding combines the conditions of persons, semantic relations between actions and objects, and spatial relations between persons and objects. We combine the three conditions into the following score function for a box $b$ with respect to action $z$:
\begin{equation}
\begin{split}
s(b, F, z) = & Pr(\texttt{person} | b) + \sum_{o \in \mathcal{O}} \Psi(o, z) \cdot \\
& \max_{b' \in o_{D}(F, b)} \bigg( Pr(o | b') \cdot \Phi(b, b', o) \bigg).
\end{split}
\label{eq:embedding}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RELATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Incorporating semantic and spatial relations}
%\label{sec:relations}
The object embedding of Equation~\ref{eq:embedding} crucially depends on two relational functions, one focusing on spatial relations ($\Phi$) and one focusing on semantic relations ($\Psi$), which will be outlined separately below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SPATIAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spatial relations between actors and objects}
\label{sec:m-spatial}
To enable localization, we emphasize the importance of a high spatial match between the actor performing the action and the object of interest. We exploit the observation that people interact with objects in preferred spatial relations. We do this by gathering statistics from the same image dataset used to pre-train the object detectors. By reusing the same dataset, we keep the amount of knowledge sources contained to a dataset for object detectors and a semantic word embedding. For the spatial awareness, we examine the bounding box annotations for the person class and all object classes. We gather all instances where an object and person box annotation co-occur. We quantize the gathered instances into representations that describe the overall spatial-awareness between people and objects.

\begin{figure}[t]
\centering
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/backpack.pdf}
\caption{Backpack.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/umbrella.pdf}
\caption{Umbrella.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/stop-sign.pdf}
\caption{Stop sign.}
\end{subfigure}
\\
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/sheep.pdf}
\caption{Sheep.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/horse.pdf}
\caption{Horse.}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=\linewidth]{images/exemplars/giraffe.pdf}
\caption{Giraffe.}
\end{subfigure}
\caption{Spatial-aware relations for six local objects. Different objects have different spatial preferences with respect to persons. We exploit this spatial awareness for zero-shot action localization.}
\label{fig:exemplars}
\end{figure}

The spatial relation between an object box relative to a person box is quantized into a 9-dimensional grid. This grid represents represents how the object box is spatially distributed to the person box with respect to the following prepositions: $\{$\emph{above left}, \emph{above}, \emph{above right}, \emph{left}, \emph{on}, \emph{right}, \emph{below left}, \emph{below}, \emph{below right}$\}$. Let $d_{1}(b, d) \in \mathcal{R}^{9}$ denote the spatial distribution of object box $d$ relative to person box $b$. Furthermore, let $d_{2}(\texttt{person}, o)$ denote the gathered distribution of object $o$ with respect to a person from the image dataset. We define the spatial relation function as:
\begin{equation}
\Phi(b, d, o) = 1 - \text{JSD}_{2}(d_{1}(b, d) || d_{2}(\texttt{person}, o)),
\label{eq:jsd}
\end{equation}
where $\text{JSD}_{2}(\cdot||\cdot) \in [0,1]$ denotes the Jensen-Shannon Divergence with base 2 logarithm. Intuitively, this function determines the extent to which the 9-dimensional distributions match. The more similar the distributions, the lower the divergence, and the higher the score according to Equation~\ref{eq:jsd}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SEMANTICS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Semantic relations between actions and objects}
\label{sec:m-semantic}
The function $\Psi(o,z)$ measures the semantic relations between object $o$ and action $z$. A standard in zero-shot literature is to embed both the action and the object into a word embedding space $\phi(\cdot)$, \eg \citep{?,?,?}. Then the semantic relation function is given as:
\begin{equation}
\Psi(o,z) = \cos(\phi(o), \phi(z)),
\end{equation}
with $\cos(\cdot,\cdot)$ the cosine similarity. While effective, this semantic setup comes with multiple persistent issues. We extend the standard semantic relation function by tackling three issues in establishing desirable semantic relations between actions and objects: semantic ambiguity, non-discriminative objects, and enforcing a bias towards basic-level objects.

\subsubsection{Semantic ambiguity}
Semantic relations between unseen actions and objects can be ambiguous, since words can have multiple meanings depending on the context. For example for the action \emph{kicking}, an object such as \emph{tie} is deemed highly relevant, because one of its meanings is a draw in a football match.  However, a \emph{tie} can also denote an entirely different object, namely a \emph{necktie}. Such semantic ambiguity leads to a focus on irrelevant objects for actions.

To combat ambiguity in the semantic relations, we empirically investigate two properties of object coherence across languages and cultures~\citep{malt1995}. First, most object categories are common across different cultures. This supports the presence of a common underlying structure, which leads to a similar formation of object categories across cultures and languages. Second, the formation of some categories can nevertheless differ among cultures, societies, or individuals. A different categorization mainly arises due to a different point of view on the utility of objects, their symbolic value, or the level of knowledge of individuals. We leverage these two properties of object coherence across languages by introducing a multi-lingual semantic similarity. For computing multi-lingual semantic representations of words at a large-scale, we are empowered by recent advances in the word embedding literature, where embedding models have been trained and made publicly available for many languages~\citep{grave2018learning}.

In a multi-lingual setting, let $L$ denote the total number of languages to use. Furthermore, let $\tau_{l}(o)$ denote the translator for language $l \in L$ applied to object $o$. Multi-lingual unseen action recognition can then be done by updating the semantic matching function as:
\begin{equation}
\Psi(o,z) = \frac{1}{L} \sum_{l=1}^{L} \cos(\phi(\tau_{l}(o)), \phi(\tau_{l}(z))).
\end{equation}
The multi-lingual semantic similarity simply states that for a high semantic match between object and action, the pair should be of a high similarity across languages. In this manner, accidental high similarity due to semantic ambiguity can be addressed, as this phenomenon is factored out over languages. Recall the example of the action \emph{kicking} and the object \emph{tie}. Contrary to English, in French, a \emph{tie} game is an \emph{\'egalit\'e} and a \emph{necktie} is a \emph{cravate}. Such a clear distinction in another language dampens the similarity with the object \emph{tie}. Moreover, this formulation enforces the correct high similarity across languages. For example, consider now the action \emph{playing the cello} and the object \emph{cello}. There is a direct correspondence between \emph{cello} in English and its translation in French \emph{violoncelle}. Including another language confirms the similarity with the object \emph{cello}.

\subsubsection{Object discrimination}
A second issue in unseen action recognition is the selection of non-discriminative objects. Only using semantic similarity to select objects ignores the fact that an object can be non-discriminative, despite being semantically similar. For example, for the action \emph{diving}, the objects \emph{person} and \emph{diving board} might both correctly be considered as semantically relevant. The object \emph{person} is however not a good indicator for the action \emph{diving}, as this object is present in many actions. The object \emph{diving board} on the other hand is a good indicator, as it is not shared by many other actions.

An organization is necessary to handle the massive number of object categories present in the real world and determine which objects have intrinsic discriminative abilities. Such an organization needs to convey the most important and discriminant information to facilitate thinking or communication with others~\citep{murphy2004big}. One particular organization is an hierarchical taxonomy~\citep{rosch1976,murphy2004big}, originally introduced by Carl Linnaeus in the 18th century for the classification of animals in biology. It relates categories by their inclusiveness: some categories are very inclusive, \eg an \emph{animal}, while others are very specific, \eg a \emph{rhesus monkey}. We are inspired by this inclusivity trade-off in object taxonomies. Similarly, in the context of unseen actions, some object categories are shared among many actions, while others are specific to only one or a few. It is desirable to select indicative objects, rather than focus on objects that are shared by many actions.

We propose a formulation to predict the relevance of every object for unseen actions. We extend the semantic relation function as follows:
\begin{equation}
\Psi_r(o, z) = \Psi(o, z) + r(o, \cdot, z),
\label{eq:semsim-p2}
\end{equation}
where $r(o, \cdot, a)$ denotes a function that estimates the relevance of object $o$ for action $z$. $r_z(o, \mathcal{Z}, z)$ denotes the relevance with respect to all actions $\mathcal{Z}$, while $r_o(o, O, z)$ the relevance with respect to the object set $O$, which we detail below.
\\\\
\textbf{Action-based object discrimination.} The taxonomic organization to describe the relations between objects and actions results in the following relevance function:
\begin{equation}
r_z(o, \mathcal{Z}, z) = \Psi(o, z) - \max_{c \in \mathcal{Z} \setminus z} \psi(o, c).
\end{equation}
Intuitively, the function $r_z(\cdot,\cdot,\cdot)$ encourages objects to be only semantically relevant for the action of interest. If the object is also relevant for other action, it is deemed less relevant for action $z$, resulting in a lower value for $\Psi_r(o, z)$.
\\\\
\textbf{Object-based object discrimination.} While the overall relations between actions and objects provides one form of taxonomy, it is also possible to investigate object discrimination solely by examining the objects themselves. We propose a second relevance function from object-object semantic relations:
\begin{equation}
r_o(o, O, z) = \Psi(o, z) - \frac{1}{|O|} \sum_{o'\in O \setminus o} \psi(o, o')^{\frac{1}{2}}.
\end{equation}
Intuitively, this relevance function promotes objects that have an intrinsically high uniqueness across the set of objects, regardless of their match to actions. The square root normalization is applied to reduce the skewness of the object set distribution.

\subsubsection{A bias towards basic-level objects}
The matching between actions and objects relies on the object categories in the set $O$. The way objects are named and categorized has an influence on their matching score. For example for the action \emph{walking with a dog}, it would be more relevant to simply name the object present in the video as a \emph{dog} rather than a \emph{domesticated animal}, or an \emph{Australian terrier}. There exists a preferred entry-level of abstraction in linguistics, for which people refer to when naming objects~\citep{jolicoeur1984pictures}. This level corresponds to the basic-level~\citep{rosch1976,rosch1988}, which is a trade-off between superordinates and subordinates. Superordinates concern broad category sets, while subordinates concern very fine-grained categories. Hence, basic-level categories are preferred because they convey the most relevant information and are discriminative from one another~\citep{rosch1976}. It has been shown that people tend to name objects by their basic-level~\citep{rosch1976}, to recognize basic-level objects faster~\citep{jolicoeur1984pictures}, and to learn them first at a young age~\citep{rosch1976}. It would then be valuable to emphasize basic-level objects rather than objects from other levels of abstraction. Here, we investigate the need for a bias towards basic-level objects for unseen actions.

To investigate which entry-level for objects is preferred, we use the relative WordNet depth of the objects in $O$ to weight each object. Intuitively, the deeper an object is in the WordNet hierarchy, the more specific the object is and vice versa. To perform the weighting, we use the beta distribution:
\begin{equation}
\begin{split}
\text{Beta}(d | \alpha, \beta) = & \frac{d^{\alpha-1} \cdot (1-d)^{\beta-1}}{B(\alpha,\beta)},\\
B(\alpha,\beta) = & \frac{\Gamma(\alpha) \cdot \Gamma(\beta)}{\Gamma(\alpha+\beta)},\\
\end{split}
\end{equation}
where $d$ denotes the relative depth of an object and $\Gamma(\cdot)$ denotes the gamma function. From the beta distribution, we use different values of the $\alpha$ and $\beta$ parameters to define different weighting philosophies.

Here, we investigate four weighting variants. The first is uniform weighting ($\alpha=1, \beta=1$), where each object receives the same weight, regardless of its WordNet depth. This is the baseline variant. The second is base-level weighting ($\alpha=2, \beta=2$), where objects with an intermediate depth receive a higher weight than the objects with the lowest depth (the most generic) and the highest depth (the most specific). We also include two extreme variants for comparison, namely a generic-focused weighting ($\alpha=1, \beta=5$), where the objects with the lowest depth receive the highest weight and a specific-focuses weighting ($\alpha=5, \beta=1$), which has the inverse effect.

The different variants result in a bias towards objects with different WordNet depths. We incorporate this in the matching by adjusting the semantic similarity function between objects and actions :
\begin{equation}
\Psi_e(o, z | \alpha, \beta) = \text{Beta}(d_o | \alpha, \beta) \cdot \Psi(o, z),
\end{equation}
where $d_o$ denotes the depth of object $o$, [0,1] normalized based on the minimum WordNet depth (2) and maximum WordNet depth (18) over all objects in $O$.

\begin{figure}[t]
\includegraphics[width=\linewidth]{images/figure-global.pdf}
\caption{Example of the action \emph{baseball swing}. Next the person (blue) swinging the baseball bat (red), there are a number of objects within the same context that help to identify the action. These include a \emph{helmet}, a \emph{baseball glove}, a \emph{home base}, and \emph{soil} (green). We incorporate information from such global objects in context to strengthen unseen action localization and classification.}
\label{fig:fig-global}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINKING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Linking action tubes}
\label{sec:m-linking}
Given scored boxes in individual frames, we link boxes into tubes to arrive at a spatio-temporal action localization. We link boxes that have high scores from our object embeddings and a have high spatial overlap. Given an action $z$ and boxes $b_{1}$ and $b_{2}$ in consecutive frames $F_{1}$ and $F_{2}$, the link score is given as:
\begin{equation}
w(b_{1}, b_{2}, z) = s(b_{1}, F_{1}, z) + s(b_{2}, F_{2}, z) + \text{iou}(b_{1}, b_{2}),
\end{equation}
where $\text{iou}(\cdot, \cdot)$ denotes the spatial intersection-over-union score. We solve the problem of linking boxes into tubes with the Viterbi algorithm~\citep{gkioxari2015finding}. For a video $V$, we apply the Viterbi algorithm on the link scores to obtain an action tube. We then remove the used boxes and their links from the video and rerun the Viterbi algorithm on the remaining links to generate a new tube. We reiterate this process until we obtain $T$ tubes. The action score $\ell_z$ for action class $z$ of an action tube $t$ is defined as the average score of the boxes in the tube:
\begin{equation}
\ell_\text{tube}(t, z) = \frac{1}{|t|} \sum_{i=1}^{|t|} s(b_{t_i}, F_{t_i}, z),
\label{eq:tubescore}
\end{equation}
where $b_{t_i}$ and $F_{t_i}$ denote respectively the box and frame of the $i^{\text{th}}$ element in $t$. For zero-shot localization, we gather tubes across all test videos and rank the tubes using the scores provided by Equation~\ref{eq:tubescore}. For zero-shot classification, we disregard the tube locations. For each video, we predict the action class label as the action with the highest tube score within the video.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GLOBAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Local- and global-aware object embeddings}
\label{sec:global}
The localized scope of the object embedding enables us to localize unseen actions spatio-temporally. Such a localized setup might however ignore relevant concepts that occur within the same scene. An example is shown for the action \emph{baseball swing} in Figure~\ref{fig:fig-global}. Several objects are present in the neighbourhood of the person swining the bat that help us in identifying the correct action. While we need an explicit focus on \emph{person} and \emph{bike} for localization, we hypothesize that incorporating global object information from context improves both the unseen action localization and classification results.

Let $\mathcal{G}$ denote a set of global object detectors that can be applied to a video. We use the global objects to obtain a global action score of a video $V$ as follows:
\begin{equation}
\ell_\text{global}(V, z) = \sum_{g \in \mathcal{G}} \Psi(g, z) \cdot p(g | V),
\end{equation}
with $p(g | V)$ the probability of global object $g$ being present in video $V$. Here, the introduced functions for the semantic relations between actions and objects can also be applied.

To combine the local and global object embeddings for unseen action localization, we simply add the global video score to each tube that is obtained from that video. Let $t$ denote a single tube from video $V$, the localization score is updated as:
\begin{equation}
\ell_\text{fusion}(t, V, z) = \ell_\text{tube}(t, z) + \ell_\text{global}(V, z).
\end{equation}
For unseen action classification, we are no longer interested in the precise localization of actions within videos. We therefore classify a video $V$ by max-pooling over the scores of the tubes within the video:
\begin{equation}
z^{\star}(V) = \argmax_{z \in \mathcal{Z}} \bigg( \max_{t \in  T_V} \ell_\text{tube}(t, z) + \ell_\text{global}(V, z) \bigg),
\end{equation}
where $T_V$ denotes the set of tubes in video $V$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RETRIEVAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Zero-shot localized action retrieval}
\label{sec:retrieval}
The use of local and global objects with the appropriate spatial and semantic awareness extends beyond unseen action localization and classification. Due to the generic setup of the approach, we can also perform a new task, dubbed zero-shot localized action retrieval. This task resembles the localization tasks, as the goal is to rank the most relevant tubes the highest. Different from localization, we now have the opportunity to specify which objects are of interest and which spatial relations are desirable for a detailed result. Furthermore, inspired by the effectiveness of size in actor-object relations~\citep{?}, we extend the retrieval setting by allowing users to specify a desired relative size between actors and objects. The ability to specify the object, spatial relations, and size allows for different localizations of the same action. To enable such a retrieval, we extend the box score function of Equation~\ref{eq:embedding} as follows:
\begin{equation}
\begin{split}
s(b, & F, o, r, s) = Pr(\texttt{person} | b) + \max_{b' \in o_{D}(F, b)}\\
& \bigg( Pr(o | b') \cdot \Phi_r(b, b', r) \cdot \big( 1 - |\frac{\text{size}(b')}{\text{size}(b)} - s| \big) \bigg),
\end{split}
\label{eq:embedding}
\end{equation}
where $o$ denote the user-specified object, $r \in \mathbb{R}^9$ the specified spatial relations, and $s$ the specified relative $s$. The spatial relation function is modified to directly match box relations to specified relations:
\begin{equation}
\Phi_r(b, d, r) = 1 - \text{JSD}_{2}(d_{1}(b, d) || r).
\end{equation}
With the three user-specified objectives, we again score individual boxes first and link them over time. The tube score is used to rank the tubes across a video collection to obtain the final retrieval result.

==> old/old-tables.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
 & \multicolumn{5}{c}{Overlap threshold}\\
 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5\\
\midrule
\rowcolor{Gray}
\textbf{UCF Sports} (AUC) & & & & &\\
\cite{jain2015objects2action} & 38.8 & 23.2 & 16.2 & 9.9 & 7.2\\
\cite{mettes2017spatial} & 43.5 & 39.3 & 37.1 & 35.7 & 31.1\\
\textit{This paper} & \textbf{47.3} & \textbf{43.0} & \textbf{40.7} & \textbf{37.9} & \textbf{33.1}\\
\midrule
\rowcolor{Gray}
\textbf{UCF Sports} (mAP) & & & & &\\
\cite{mettes2017spatial} & 47.4 & 43.5 & 42.1 & 32.0 & 23.2\\
\textit{This paper} & \textbf{61.2} & \textbf{54.2} & \textbf{54.0} & \textbf{41.5} & \textbf{34.9}\\
\midrule
\rowcolor{Gray}
\textbf{J-HMDB} (AUC) & & & & &\\
\cite{mettes2017spatial} & 34.6 & 33.3 & 30.5 & 26.8 & 23.0\\
\textit{This paper} & \textbf{37.3} & \textbf{37.1} & \textbf{33.9} & \textbf{31.0} & \textbf{26.7}\\
\midrule
\rowcolor{Gray}
\textbf{J-HMDB} (mAP) & & & & &\\
\cite{mettes2017spatial} & 27.5 & 27.0 & 23.2 & 19.2 & 15.1\\
\textit{This paper} & \textbf{32.1} & \textbf{31.5} & \textbf{27.2} & \textbf{22.6} & \textbf{17.6}\\
%\midrule
%\rowcolor{Gray}
%\textbf{Hollywood2ubesT} (AUC) & & & & &\\
%\cite{mettes2017spatial} & 21.0 & 13.8 & 8.6 & 4.7 & 0.2\\
%\textit{This paper} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\bottomrule
\end{tabular}
}
\caption{Unseen action localization comparisons to~\cite{mettes2017spatial} on UCF Sports using AUC and mAP as metrics and J-HMDB using AUC. Across all comparisons, we obtain improved results, indicating the effectiveness of our approach.}
\label{tab:sota-localization-2}
\end{table}

==> old/relatedwork-old.tex <==
\section{Related work}
\label{sec:related}

\subsection{Zero-shot action classification}
For zero-shot action classification, a common approach is to generalize from seen to unseen actions by mapping videos to a shared attribute space~\citep{}, akin to attribute-based approaches in images~\citep{}. Attribute classifiers are trained on seen actions and applied to test videos. The obtained attribute classifications are in turn compared to a priori defined attribute annotations for unseen actions. The attribute-based approach has been extended by using knowledge about test video distributions in transductive settings~\citep{} and by incorporating domain adaptation~\citep{}. \psmm{CVPR18 here?} Since attributes are a priori defined from expert knowledge, this setting does not generalize to arbitrary zero-shot queries. Furthermore, the attributes are globally defined, making localization impossible. Hence we refrain from employing attributes.

Several works have investigated skipping the mapping to attributes and directly map unseen actions to seen actions. \cite{li2016recognizing} map features from videos to a semantic space shared by seen and unseen actions, while \cite{gan2016recognizing} train a classifier for unseen actions by performing several levels of relatedness it to seen actions. While eliminating the need for attributes, this line of work still requires videos of seen actions to train models and are limited to classification. We focus on localization and classification, without the need for any video example to train on.

A number of works have also investigated the zero-shot classification in videos from object classification scores. In action recognition several works have investigated the use of objects by performing a semantic matching through word vectors~\citep{} or auxiliary textual descriptions~\citep{}. A similar trend occurs in zero-shot event detection from objects~\citep{}. The use of objects allows for a generalization to arbitrary unseen actions. Still however, these approaches compute scores globally for videos, restricting their use to classification. In this work, we take the object-based perspective to a local level by modeling the spatial relations between actors and objects, allowing us to perform action localization, classification, and retrieval. We furthermore improve the semantic matching between actions and objects, which benefits any object-based action recognition without examples.

Recently, \psmm{CVPR19 + related}

\subsection{Zero-shot action localization}
Spatio-temporal localization of actions without examples is hardly investigated in current literature. A notable exception is the work of~\cite{jain2015objects2action}, which has an experiment on zero-shot action localization from objects. This setup is however limited in two aspects. First, it is computationally expensive. Each test video is split into spatio-temporal proposals based on~\citep{jain2017tubelets}. Then for each proposal, boxes are sampled and individually fed to a pre-trained object classification network to obtain object scores. The object scores of each proposal are semantically matched to the action and the best matched proposal is selected as the location of interest. This setup requires in the order of $10^4$ forward passes for a pre-trained convolutional network to obtain object scores in one video. A second limitation is that~\cite{jain2015objects2action} assume that objects occur \emph{on} the actor when performing an action. In this paper, we employ local object detectors and embed spatial relations between actors and objects, resulting in a better and more practical zero-shot action localization.

\subsection{Action-object relations}
For our unseen action localization and classification, we are empowered by multiple works that highlight the strong match between actions and objects. \psmm{Highlight these works.} \psmm{Include actor-object relation classification in images?}
